Detection and Impact of Debit/Credit Card Fraud: Victims' Experiences

It might be intuitive to expect that small or reimbursed financial loss resulting from credit or debit card fraud would have low or no financial impact on victims. However, little is known about the extent to which financial fraud impacts victims psychologically, how victims detect the fraud, which detection methods are most efficient, and how the fraud detection and reporting processes can be improved. To answer these questions, we conducted a 150-participant survey of debit/credit card fraud victims in the US. Our results show that significantly more participants reported that they were impacted psychologically than financially. However, we found no relationship between the amount of direct financial loss and psychological impact, suggesting that people are at risk of being psychologically impacted regardless of the amount lost to fraud. Despite the fact that bank or card issuer notifications were related to faster detection of fraud, more participants reported detecting the fraud after reviewing their card or account statements rather than from notifications. This suggests that notifications may be underutilized. Finally, we provide a set of recommendations distilled from victims' experiences to improve the debit/credit card fraud detection and reporting processes.

==> misc/ARCHIVE_old_tables.tex <==
\begin{comment}
\begin{table}[t!]
    \footnotesize
    \centering
    \caption{Pairwise Chi-squared tests for the financial vs. psychological vs. trust impacts. The p-values were adjusted using the Bonferroni method. The chi-squared effect size was computed using Cramer's V ($\alpha_c$) for significant results.}
    \label{tab:fin_vs_psych_vs_trust}
    %\resizebox{0.75\columnwidth}{!}{
    \begin{tabular}{l|l|l|l}
    \toprule
    \multicolumn{4}{c}{\textit{N = 150}} \\
    \midrule
    Impacted (at time)  &  $\chi^2(2)$    &  \makecell{Adjusted\\p-value}     &   $\alpha_c$   \\
    \hline 
    Fin. vs. Psych.     & 23.413          & \cellcolor{gray!30}< .001   & 0.272 \\
    Fin. vs. Trust      & 21.067          & \cellcolor{gray!30}< .001  & 0.258  \\
    Psych. vs. Trust    & 0.068           & .794                        & n.a. \\                    
    \midrule 
    Impacted (today)    &  $\chi^2(2)$    &  \makecell{Adjusted\\p-value}    &   $\alpha_c$   \\
    \hline 
    Fin. vs. Psych.     & 17.084          & \cellcolor{gray!30}< .001  & 0.230 \\
    Fin. vs. Trust      & 52.983          & \cellcolor{gray!30}< .001  & 0.413  \\
    Psych. vs. Trust    & 11.327          & \cellcolor{gray!30}< .001  & 0.187  \\  
    \bottomrule
    \end{tabular}
    %} %  end resizebox
\end{table}
\end{comment}
